How Can Everyday Users Efficiently Teach Robots by Demonstrations?

Learning from Demonstration (LfD) is a framework that allows lay users to easily program robots. However, the efficiency of robot learning and the robot's ability to generalize to task variations hinges upon the quality and quantity of the provided demonstrations. Our objective is to guide human teachers to furnish more effective demonstrations, thus facilitating efficient robot learning. To achieve this, we propose to use a measure of uncertainty, namely task-related information entropy, as a criterion for suggesting informative demonstration examples to human teachers to improve their teaching skills. In a conducted experiment (N=24), an augmented reality (AR)-based guidance system was employed to train novice users to produce additional demonstrations from areas with the highest entropy within the workspace. These novice users were trained for a few trials to teach the robot a generalizable task using a limited number of demonstrations. Subsequently, the users' performance after training was assessed first on the same task (retention) and then on a novel task (transfer) without guidance. The results indicated a substantial improvement in robot learning efficiency from the teacher's demonstrations, with an improvement of up to 198% observed on the novel task. Furthermore, the proposed approach was compared to a state-of-the-art heuristic rule and found to improve robot learning efficiency by 210% compared to the heuristic rule.

==> Text/objective.tex <==
The objective of this research is to help human teachers provide demonstrations efficiently by using information entropy as the criterion for selecting demonstrations for robot learning and generalization. Furthermore, we propose integrating Augmented Reality (AR) with the entropy-based guidance system as a training framework to help novice users learn to better identify informative demonstrations which favour undemonstrated states and avoid ambiguous demonstrations. Finally, we compare two visualization techniques to help users provide an efficient set of demonstrations for the robot to learn from. The research questions we seek to answer are as follows:
\begin{enumerate}
  \item Does information entropy improve robot learning efficiency through driving demonstration selection?
  \item Does an entropy-based guidance system improve users' performance in teaching robots by demonstration?
  \item How much visual information should be provided in the guidance system to improve the user's teaching efficiency? 
  \item How much visual information should be provided in the guidance system to improve the user's teaching efficiency in transfer test?
\end{enumerate}


To answer the first question, we compared an entropy-based guidance system to a heuristic guidance system proposed in~\cite{sena2020quantifying} and evaluated the robot learning efficiency in simulation. The heuristic rule's steps are: (i) provide one demonstration, starting from anywhere in the task space, (ii) continue providing demonstrations within 4 cm of the first demonstration, until the first demonstration is surrounded by successful test points, (iii) provide further demonstrations within 4 cm of the successful test points, in the area with the greatest number of failed test points, till generalize to all test point successfully. To answer the second question, we integrated the proposed entropy-based guidance system in a training framework for novice users to see if their teaching skills (in terms of the number and the distribution of the provided demonstrations) improved after training. To answer the third question, we conducted a user study to compare two visual guidance systems: 1) single point suggestion and 2) a heatmap representation of the task space's entropy values. The comparison aims to determine the relationship between the amount of visual information provided to the users and their resulting teaching efficiency. This comparison is evaluated on a trained task (i.e., retention test) and in a new task (i.e., transfer test) to address the fourth question. An overview of the user study is detailed in fig.~\ref{fig:training} and the experimental setup used in the user study is shown in fig.~\ref{fig:exp_setup}



% To answer these questions, we first compared an entropy-based guidance system to a heuristic guidance system proposed in~\cite{sena2020quantifying} in terms of robot learning efficiency in simulation. The demonstrations used in the simulation are from a motion planner and from a human teacher (one of the paper's authors). Then, we conducted a user study to compare two visual guidance systems: 1) single point suggestion and 2) a heatmap representation of the task space's entropy values. The comparison aims to determine the relationship between the amount of visual information provided to users and the users' resulting teaching efficiency. Specifically, we want to see how much undemonstrated states are favoured and ambiguous demonstrations are avoided after using each of the visual guidance systems. This comparison is evaluated on a trained task (i.e., retention test) and in a new task (i.e., transfer test). 



==> Text/system.tex <==
\subsection{System Overview}
Our experimental system comprises three key components: the robot, its programming interface, and the visual interface. The robot is a KUKA IIWA LBR14 robot mounted in an inverted position on a two-axis movable platform. This robot features impedance control capabilities, making it suitable for tasks involving physical contact with the environment and safe interaction with humans. To facilitate these tasks, we equipped the robot with a simple spring-loaded end-effector holding a marker pen, as depicted in Figure~\ref{fig:exp_setup}. A whiteboard was placed beneath the robot and will be used in the experimental task described in Section~\ref{subsec:task}. 

To program the robot's motion, We implemented a joystick interface using a standard PS3 joystick to program the robot's motion, mimicking teaching pendants' functionalities. Users use the joystick to control the end-effector's positioning. At the start of each demonstration, a specific button moves the robot to a safe height, and users can manipulate the end-effector. Another button saves the trajectory data, which is then sent to the control computer. Pressing the clear button resets the trajectory and clears saved points. 

The visual interface system comprises a Microsoft HoloLens AR head-mounted display~\cite{kress201711} and the ROS Bridge communication library \cite{rosbridge}. The AR interface is developed using Unity and the ROS\# programming library~\cite{ros-sharp}. This setup allows for the rendering of 3D AR displays and user interface elements co-located with the real robot and workspace. During operation, the AR system overlays a geometrically accurate starting zone on the real environment, offering user feedback on the robot's progress and guiding efficient demonstration, as shown in Figure~\ref{fig:overview}. Calibration is achieved through a fiducial marker (ARTag), and the virtual models provide task context and visual feedback, with the option for precise alignment using voice commands.

The control computer processes user commands, handles trajectory learning, inverse kinematics, and sends low-level commands to the real robot for motion execution. These functionalities are implemented using the Robot Operating System (ROS). Data communication between the HoloLens and the control computer is facilitated by the ROS Bridge communication library over a wireless connection, managing data format translation. The joystick connects to the control computer via a USB cable.

\subsection{Robot Task Learning}
\label{sec:learning}

A task parameterized Gaussian Mixture Model (TP-GMM) combined with Gaussian Mixture Regression (GMR) is used for task learning. TP-GMMs have been extensively used for LfD~\cite{pervez2018learning, osa2018algorithmic}, and they show good generalization using a limited set of demonstrations. TP-GMMs model a task with parameters that are defined by a sequence of coordinate frames. In a \(D\) dimensional space, each task parameter/coordinate frame is given by an $A \in \mathbb{R}^{D \times D}$ matrix indicating its orientation and a $b \in \mathbb{R}^D$ vector indicating its origin, relative to the global frame. A \(K\)-component mixture model is fitted to the data in each local frame of reference. Each GMM is described by $\left(\pi_k, \mathbf{\mu}^{(j)}_k, \mathbf{\Sigma}^{(j)}_k\right)$, referring to the prior probabilities, mean, and covariance matrices for each component \(k\) in frame \(j\), respectively.

A Bayesian Information Criterion (BIC) was used to define the optimal number of \(K\)-Gaussian components to fit the demonstrations. In addition, an expectation-maximization (EM) algorithm is used to estimate these parameters, with the constraint that data points from different frames of reference must arise from the same source. To use the local models for trajectory generation, they must be projected back into the global frame of reference and then combined into one global model. This is achieved through a linear transformation of the local models with their respective task parameters, followed by a product of Gaussians. The new GMM components $\left\{\pi_k, \mathbf{\mu}_{k,t}, \mathbf{\Sigma}_{k,t} \right\}_{k=1}^K$ at time $t$ in the global frame $\left\{O \right\}$ can be computed as:
\begin{equation}
    \mathcal{N}\left(\boldsymbol{\mu}_{k,t}, \boldsymbol{\Sigma}_{k,t} \right) \propto \prod^J_{j=1} \mathcal{N}\left(\mathbf{A}_t^{(j)} \boldsymbol{\mu}_k^{(j)} + \mathbf{b}_t^{(j)}, \mathbf{A}_t^{(j)} \boldsymbol{\Sigma}_k^{(j)} (\mathbf{A}_t^{(j)})^T \right)
\end{equation}

Then, GMR can be used to obtain the next trajectory point. This procedure is repeated for each time step in the trajectory. Calinon \cite{calinon2016tutorial} provides further details.





